Generalizable Long-Horizon Manipulations with Large Language Models

This work introduces a framework harnessing the capabilities of Large Language Models (LLMs) to generate primitive task conditions for generalizable long-horizon manipulations with novel objects and unseen tasks. These task conditions serve as guides for the generation and adjustment of Dynamic Movement Primitives (DMP) trajectories for long-horizon task execution. We further create a challenging robotic manipulation task suite based on Pybullet for long-horizon task evaluation. Extensive experiments in both simulated and real-world environments demonstrate the effectiveness of our framework on both familiar tasks involving new objects and novel but related tasks, highlighting the potential of LLMs in enhancing robotic system versatility and adaptability. Project website: https://object814.github.io/Task-Condition-With-LLM/

==> tex/reproduction.tex <==
\begin{figure*} [!t]
    \centering
    \includegraphics[width=\textwidth]{img/Figure2.png}
    \caption{Task execution Structure} \my{TODO: more caption and change figure name}
    \label{fig:repro_structure}
\end{figure*}

The structure of task reproduction under task condition constraint is shown in Fig.2. Three main functions are used sequentially to achieve primitive task reproduction while gathering data from both the environment and previous demonstrations. In order to test the framework's ability in task condition generalization using the LLM, we designed two sets of reproduction experiments, which are demonstrated task reproduction and unseen task reproduction. These two sets of reproduction experiments will only have differents 

\subsection{Task Condition Generalization Using LLM}
The definition and components of a task condition are the same as mentioned in \S V.A. and we use two LLM chats to do task condition generalization as well. The examples in prompts given to the LLM will now be the successfully generated task conditions during demonstrations.

It's obvious that if the kind of primitive task we wish to reproduce already exists in the examples, such as, we wish to generalize task condition for 'grasp mug' given example of 'grasp bottle', the LLM will perform in the same way as task condition generation in \S V.A. The difference will occur when we give the LLM a kind of reproduction task that does not exist in examples. We wish it can learn from the examples and generalize reasonable spatial relations and object states for the unseen task, and keep the output in the same format. Therefore, the prompt for generalization adds the chain of thoughts on what to do, the meaning of pre/post conditions, and a rule to regulate output format based on task condition generation in \S V.A. The prompt given to the LLM for spatial relations generalization is as below, and the prompt used to do object states generalization has a consistent structure therefore we are not showing it here.

\begin{tcolorbox}[width=0.48\textwidth, colframe=gray, left=0pt, right=0pt, top=0pt, bottom=0pt, size=minimal]
\vspace{.05in}
\footnotesize
I wish you to be a spatial relations and collisions judgment machine.\\
\textcolor{violet}{I will give you a task name describing a manipulator task. The end effector of the manipulator is a gripper.}\\
\textcolor{violet}{First, you should determine what are the relevant objects in this task}.\\
\textcolor{violet}{Then, you should present what spatial relations these objects should have before (pre-conditions) and after (post-conditions) the task is processed.}\\
\textcolor{violet}{Keep in mind that before the task is processed, the task itself is not satisfied.}\\
\textcolor{violet}{After the task is processed, the task is satisfied.}\\
\textcolor{blue}{Here are the spatial relations you can choose from:}\\
\textcolor{blue}{above, below, inside, in front of}\\
\textcolor{violet}{At last, you should present what collisions there might occur during the completion of the task. You must only generate collisions that includes the relevant objects.}\\
\textcolor{orange}{Here are some examples:}\\
\textcolor{orange}{{[} Examples of task condition with only spatial relations and collisions {]}}\\
\textcolor{violet}{Remember to strictly follow the examples' format, and do not generate any pre/post conditions except spatial relations I gave you to choose from.}\\
\textcolor{teal}{Q: Task name: {[}Reproduction Task Name{]}}
\vspace{.05in}
\\ \my{caption?}
\end{tcolorbox}

\subsection{Trajectory Generation Using DMP And Manipulator Controlling}

With learned DMP trajectory parameters from \S V.B for each primitive task, we can generate trajectories with a similar shape as the demonstration trajectory by getting the nonlinear term \(f\) described in (5) using starting position \(y_0\) and goal position \(g\). Then, we can get the position \(y\) and its first and second derivatives by running numerical simulation of the second order system (1). Though the trajectory generated in this way will be relevant to the variable \(x\) instead of time, we manage to record the lasting time of the demonstration trajectory by multiplying step number with sample frequency, and while reproducing the new trajectory, we can just calculate the number of steps we need given a desired lasting time and reproducing frequency. Then do interpolation or sampling to make it that length.

As for manipulator controlling, we give Pybullet the end effector trajectory including position and orientation, while ensuring it is dense enough to avoid large acceleration or velocity. Then we call the built-in inverse kinematic function of Pybullet to calculate joint positions and do position controlling. Though straightforward, this controlling method is stable enough for our experiments.

\subsection{Trajectory Generation With Task Condition}

With the corresponding task condition generalized by the LLM, we set up a task reproduction method with task condition constraining the movement in order to evaluate the role of it during reproduction, and whether it can boost up the success rate of a long horizon task. There are two steps included in our method, which are pre-condition satisfaction and trajectory reproduction with condition.

The pre-condition satisfaction, as the name goes, is conducted before reproducing a primitive task, and is aimed to satisfy the pre-conditions of the task before operation. To achieve this, a recursive algorithm is used and its pseudo code is shown in algorithm 1. 

\begin{algorithm}
\caption{Pre-Condition Satisfaction}
\label{alg: Task condition satisfy}
\begin{algorithmic}[1]
\Require
\Statex \textit{T\_Cond} - \textbf{T}ask Condition
\Ensure{None} 
\Function {\colorbox[RGB]{224,224,224}{SatisfyPreCond}}{\textit{T\_Cond}}
    \State \textit{currentConds} $\gets$ \textproc{FromEnvPC}(\textit{})
    \State \textit{preConds} $\gets$ \textproc{FromCond}(\textit{T\_Cond})
    \For {\textit{preCond} \textbf{in} \textit{preConds}}
        \If {\textit{preCond} \textbf{not in} \textit{currentCond}}
            \State \textit{newT\_Name} $\gets$ \textproc{Cond2Task}(\textit{preCond})
            \State \textit{newT\_Cond} $\gets$ \textproc{GenCond}(\textit{newT\_Name})
            \State \textproc{\colorbox[RGB]{224,224,224}{SatisfyPreCond}}
            (\textit{newT\_Cond})
            \State \textproc{ControlWithCond}(\textit{newT\_Cond})
        \EndIf
        \If {\textit{RUNTIME} $>$ 3*\textit{taskTime}}
            \State break
        \EndIf
    \EndFor
\EndFunction
\end{algorithmic}
\end{algorithm}

Given the reproduction task condition, the algorithm gets the pre-conditions in it and compares them to the current conditions in the environment, which are acquired using the same method mentioned in \S V.A. Then, the pre-conditions that are not currently satisfied will raise a primitive task aiming to satisfy it, which is represented as Cond2Task function in algorithm 1. The mapping between conditions and primitive tasks is done by human, for example, if the pre-condition 'gripper grasping bottle' is not satisfied, the primitive task 'grasp bottle' will be the new task name in the algorithm, and its pre-condition will be generated and satisfied in the same way. Only when all pre-conditions are satisfied or the total running time exceeds 3 times the recorded running time during demonstration will the system move on to controlling the robot.

After pre-condition satisfaction, we move on to trajectory reproduction with condition. It is aimed to avoid unwanted collisions during reproduction and help correct the trajectory generated by the DMP. The pseudo code is shown in algorithm 2. 

\begin{algorithm}
\caption{Trajectory Reproduction With Condition}
\label{algo:control_manipulator}
\begin{algorithmic}[1]
\Require{\textit{T\_Cond} - \textbf{T}ask Condition}
\Ensure{None}
\Function{ControlWithCond}{\textit{T\_Cond}}
\State \textit{taskTime, taskColl, post-conditions} $\gets$ FromCond(\textit{T\_Cond})
\State \textit{targetPos} $\gets$ FromEnvPC()
\State \textit{goalPos} $\gets$ \textit{targetObjPos}
\State \textit{trajDMP}[:] $\gets$ GenDMP(\textit{goalPos})
\While {\textit{RUNTIME} $\leq$ 3*\textit{taskTime} \textbf{or} end(\textit{trajDMP}) \textbf{or} post-conditions satisfied} 
    \State ControlManipulator(\textit{trajDMP}[+1])
    \State \textit{currentColl} $\gets$ FromEnvPC()
    \If {\textit{currentColl} not in \textit{taskColl}}
        \State ControlManipulator(\textit{trajDMP}[-10])
        \State \textit{collPos} $\gets$ FromEnvPC()
        \State \textit{goalPos} $\gets$ \textit{goalPos} + (\textit{goalPos} - \textit{collPos})
        \State \textit{trajDMP}[:-1] $\gets$ GenDMP(\textit{goalPos})
    \EndIf
\EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}


